Using Automatically Extracted Minimum Spans to Disentangle Coreference Evaluation from Boundary Detection

The common practice in coreference resolution is to identify and evaluate the maximum span of mentions. The use of maximum spans tangles coreference evaluation with the challenges of mention boundary detection like prepositional phrase attachment. To address this problem, minimum spans are manually annotated in smaller corpora. However, this additional annotation is costly and therefore, this solution does not scale to large corpora. In this paper, we propose the MINA algorithm for automatically extracting minimum spans to benefit from minimum span evaluation in all corpora. We show that the extracted minimum spans by MINA are consistent with those that are manually annotated by experts. Our experiments show that using minimum spans is in particular important in cross-dataset coreference evaluation, in which detected mention boundaries are noisier due to domain shift. We will integrate MINA into https://github.com/ns-moosavi/coval for reporting standard coreference scores based on both maximum and automatically detected minimum spans.

==> mina_acl2019/add.tex <==
\paragraph{When MINA fails due to parsing errors}

\begin{figure}
\centering
 \resizebox{\columnwidth}{!}{\Tree [.NP " [.NP Jingle Babies ] , " and , [.PP of [.NP course ]] , " [.NP Jingle Dogs ]]}
\caption{.\label{pp}}
\end{figure}

\begin{figure}
\centering
 \resizebox{\columnwidth}{!}{\Tree [.FRAG [.NP " [.NP Jingle Babies ] , " and , [.PP of [.NP course ]]] , " [.NP Jingle Dogs ] . " ]}
\caption{.\label{pp}}
\end{figure}

\begin{figure}
\centering
 \resizebox{\columnwidth}{!}{\Tree [.NP [.NP Ben Ginsberg ][.NP [.NP attorney ][.PP for [.NP [.NP the Bush team ][.PRC [.ADJP victorious ][.NP today][.PP in [.NP Tallahassee ]]]]]]]}
\caption{.\label{pp}}
\end{figure}

\begin{figure}
\centering
 \resizebox{\columnwidth}{!}{\Tree [.FRAG [.NP [.NP Ben Ginsberg ][.NP [.NP attorney ][.PP for [.NP the Bush team ]]]][.NP victorious today ][.PP in [.NP Tallahassee ]]]}
\caption{.\label{pp}}
\end{figure}

==> mina_acl2019/analysis.tex <==
\section{Analysis}
In order to better understand the impact of using minimum spans in cross-dataset evaluations, we analyze the output of \texttt{deep-coref RL}, on which minimum span evaluation has the largest impact, for the cases in which a system mention and its corresponding gold mention have the same minimum span while they have different maximum boundaries.

We have included some examples from these mismatches in Example~\ref{appositive}--Example~\ref{last}.
The boundaries of gold and system mentions are determined by $g$ and $s$ indices, respectively. Mismatching spans are boldfaced in all examples.

We observe that the majority of the mismatches are due to (1) incorrect detection of appositive relation (Example~\ref{appositive}), (2) mismatch as a result of not including a surrounding quotation (Example~\ref{quotation}), and (3) inclusion of an additional comma at the end of the mention (Example~\ref{comma}).

\begin{example}
 Canada is noted for having a positive relationship with [[the Netherlands]$_g$\textbf{, owing,}]$_s$ in part, to its contribution to the Dutch liberation during World War II.
 \label{appositive}
\end{example}

\begin{example}
 .[[Le Courrier du Sud]$_g$\textbf{,}]$_s$ published by Quebecor Media, is the oldest, and contains inserts tailored to specific boroughs
 \label{comma}
\end{example}

\begin{example}
in 2007, [[Pierce College]$_g$ \textbf{sheltered}]$_s$ and fed more than 150 horses under the direction of the L.A. County Volunteer Equine Response team.
\end{example}

\begin{example}
Prime Minister Brian Mulroney's Progressive Conservatives abolished the NEP and changed the name of FIRA to [\textbf{``}[Investment Canada]$_s$\textbf{''}]$_g$, to encourage foreign investment.
\label{quotation}
\end{example}

\begin{example}
In 2011, [$_s$\textbf{nearly 6.8 million} [$_g$Canadians]] listed a non-official language as their mother tongue.
\label{last}
\end{example}

%It is worth noting that a coreference resolver can benefit a downstream application by determining all pieces of the context that are related to the entity\footnote{E.g., for answering a question about that entity}, or by disambiguation of pronouns\footnote{E.g., to correctly translate pronouns in languages with grammatical gender}.


==> mina_acl2019/conc.tex <==
\section{Conclusions}
Coreference evaluation based on maximum spans directly penalizes coreference resolvers because of parsing complexities and also small noises in mention boundary detection.
This is a known problem that is addressed by manually annotating minimum spans as well as maximum spans in several corpora.
Minimum span annotation is expensive, and therefore 
it is not a scalable solution for large coreference corpora.
In this paper, we propose the \mina algorithm to automatically extract minimum spans
without introducing additional annotation costs.
\mina automatically extracts corresponding minimum spans for both gold and system mentions and uses the resulting minimum spans in the standard evaluation metrics.
Based on our analysis on the MUC and ARRAU datasets, 
extracted minimum spans are compatible
with those that are manually annotated by experts.
The incorporation of automatically extracted minimum spans reduces the effect of maximum boundary detection errors in coreference evaluation and results in a fairer comparison.
Our results show that the use of minimum spans in coreference evaluation is of particular importance for cross-dataset settings, in which the detected maximum boundaries are noisier.

In addition to coreference evaluation, automatically extracted minimum spans can benefit 
the annotation process of new corpora.
If we provide automatically extracted minimum spans alongside maximum spans to the annotators,
the annotation of coreference relations may get easier.
For instance, detecting the coreference relation of the two nested mentions in ``[a deutsche mark based currency board where we have a foreign governor on [the board]$_{(1)}$]$_{(1)}$''\footnote{Taken from the CoNLL-2012 development set.}
would be more straightforward knowing that the minimum span of the first mention is ``a currency board''.
%\begin{example}
%In Pleasant Grove we recently met [these three sisters all in [their]$_{(1)}$ eighties 
%who have high hopes that the frozen airman proves to be [their]$_{(1)}$ big brother Glen Munn whose plane went missing in the Sierra back in nineteen forty-two]$_{(1)}$   
%\end{example}
%\begin{example}
% It's a far cry from the previous treatment of [the network, which had to overcome jamming of [its]$_{(1)}$ frequencies and intimidation of local correspondents 
% (who filled reports to [the network]$_{(1)}$ by phone, secret messengers or letters).]$_{(1)}$
%\end{example}

A future direction is to investigate the effect of using \mina spans not only in evaluation but also for training existing coreference resolvers. Maximum spans are recoverable given the \mina spans and their corresponding parse trees. Therefore, we can use \mina spans for training and testing coreference models and then retrieve their corresponding maximum spans for evaluation.
Investigating the use of \mina in other NLP areas, e.g., evaluating spans in named entity recognition or reading comprehension, is another future line of work.

 


==> mina_acl2019/coref_effect.tex <==

\begin{table*}[htbp]
    \begin{center}%\footnotesize
    %\resizebox{\columnwidth}{!}{%
	   \begin{tabular}{l|lll||lll}
	  \multicolumn{1}{c}{} & \multicolumn{3}{c}{CoNLL} & \multicolumn{3}{c}{LEA}\\  
	  \multicolumn{1}{c}{} & max & \mina & head & max & \mina & head \\
	 %\multicolumn{1}{c}{} & \multicolumn{2}{c}{max span} & \multicolumn{2}{c}{MINA-gold} & \multicolumn{2}{c}{MINA-sys}\\
     %& CoNLL & LEA & CoNLL & LEA  & CoNLL & LEA\\
     \hline
    %gold & $100$ & $100$ & $99.98$ & $99.95$ & $99.93$ &  $99.85$ \\
     \multicolumn{1}{c}{} &  \multicolumn{6}{c}{CoNLL-2012 test set} \\ \hline
    Stanford rule-based & $55.60$ (8) & $57.55$ (8)& $57.38$ (8) & $47.31$ (8) & $49.65$ (8) & $49.44$ (8)\\
     %Durret13 & $61.24$ & $62.96$ & $62.86$ & $54.00$ & $56.09$  & $55.95$\\
     cort & \cellcolor{blue!10}$63.03$  (7)& \cellcolor{blue!10}$64.60$ (6)& $64.51$ (6) & $56.10$  (6)& $58.05$ (6)& $57.93$ (6)\\ 
    Peng et al. & \cellcolor{blue!10}$63.05$ (6)& \cellcolor{blue!10}$63.50$ (7)& $63.54$ (7)& $55.22$ (7) & $55.76$ (7) & $55.80$ (7)\\ 
     %Wiseman15  & $63.40$ & $65.09$ & $65.01$ & $56.48$  & $58.57$  & $58.47$\\ 
     %W\&R16 & $64.21$ & $57.71$ & $66.04$ & $59.98$ & $66.00$ & $59.90$\\
     deep-coref ranking & $65.59$ (5) & $67.29$ (5)& $67.09$ (5)& $59.58$ (5) & $61.70$ (5) & $61.43$ (5)\\
     deep-coref RL & $65.81$ (4) & $67.50$ (4)& $67.36$ (4)& $59.76$ (4) & $61.84$  (4)& $61.64$ (4)\\
     %Lee17-single & $67.23$ & $61.24$ & $68.62$ & $62.93$\\
     Lee et al. 2017 single & $67.23$ (3) & $68.55$ (3) & $68.53$ (3) & $61.24$ (3)& $62.87$  (3)& $62.82$ (3)\\
     Lee et al. 2017 ensemble & $68.87$ (2)  & $70.12$ (2) & $70.05$ (2) & $63.19$ (2) & $64.76$ (2)& $64.64$ (2)\\
	 Lee et al. 2018 & $72.96$ (1) & $74.26$ (1)& $75.29$ (1)& $67.73$ (1) & $69.32$ (1)& $70.40$ (1)\\
     %Lee18 & $72.28$ & $73.67$ & $73.61$ & $66.89$  & $68.64$  & $68.51$\\
     \hline
     \multicolumn{1}{c}{} &  \multicolumn{6}{c}{WikiCoref} \\ \hline
     Stanford rule-based & \cellcolor{blue!10}$51.78$ (4)& \cellcolor{blue!10}$53.79$ (5)& $57.10$ (4) & \cellcolor{blue!10}$43.28$ (5)  & \cellcolor{blue!10}$45.48$ (6) & $49.28$ (4)\\
     deep-coref ranking & \cellcolor{blue!10}$52.90$ (3) & \cellcolor{blue!10}$55.16$ (2) &$57.13$ (3)& $44.40$ (3)  & $46.98$ (3) & $49.05$ (5)\\
     deep-coref RL & \cellcolor{blue!10}$50.73$ (5) & \cellcolor{blue!10}$54.26$ (4)& $57.16$ (2)& \cellcolor{blue!10}$41.98$ (6)  & \cellcolor{blue!10}$46.02$ (4)& $49.29$ (3)\\
	 Lee et al. 2017 single & $50.38$ (6) & $52.16$ (6)& $54.02$ (6) & \cellcolor{blue!10}$43.86$ (4) & \cellcolor{blue!10}$45.75$ (5) & $47.69$ (6)\\
	 Lee et al. 2017 ensemble & \cellcolor{blue!10}$53.63$ (2) & \cellcolor{blue!10}$55.03$ (3) & $56.80$ (5) & $47.50$ (2)  & $48.98$ (2) & $50.87$ (2)\\
	 Lee et al. 2018 & $57.89$ (1) & $59.90$ (1) & $61.33$ (1)& $52.42$ (1) & $54.63$ (1) & $56.19$ (1)\\
    \end{tabular}
   %}
    \end{center}
    \caption{Evaluations based on maximum span, \mina, and head spans on the CoNLL-2012 test set and WikiCoref. The ranking of corresponding scores is specified in parentheses. Rankings which are different based on maximum vs. \mina spans are highlighted.}
    \label{tab:state_of_the_art}
\end{table*}

\section{Effect on Coreference Evaluation}
\label{ch:mint:analysis}
\subsection{Experimental Setup}
In this section, we investigate how the use of minimum spans instead of maximum spans in coreference evaluation affects the results in in-domain as well as cross-dataset evaluations.
For comparisons, we use the 
\emph{CoNLL} score \cite{pradhan14},
i.e.\ the average F$_1$ value of \emph{MUC} \cite{vilain95}, \emph{B}$^3$ \cite{bagga98b},
and \emph{CEAF}$_e$ \cite{luoxiaoqiang05a}, and the \emph{LEA} F$_1$ \cite{moosavi16b} score.\footnote{We use the python implementation that is available at \url{https://github.com/ns-moosavi/coval}.}  
%of the participating systems in the CoNLL 2012 shared task (closed task with predicted syntax and mentions) based on both maximum and minimum span evaluations.
Minimum spans are detected using both \mina and Collins' head finding rules.
All examined coreference resolvers are trained on the CoNLL-2012 training data.
For in-domain evaluations, models are evaluated on the CoNLL-2012 test data and minimum spans are extracted using gold parse trees, which are provided in CoNLL-2012.\footnote{We also examined the in-domain results of Table~\ref{tab:state_of_the_art} based on the system parse trees of CoNLL-2012 instead of gold parse trees. The differences between scores based on \mina spans that are extracted from gold vs.\ those that are extracted from system parse trees were only about 0.2 points.}

For cross-dataset evaluations, models are tested on the WikiCoref dataset \cite{ghaddar16b}.
For extracting minimum spans, we parse WikiCoref by the Stanford neural parser.
%The results on WikiCoref represents a cross-dataset evaluation setting: all systems are trained on CoNLL-2012 and tested on WikiCoref.
This dataset is annotated using the same annotation guidelines as that of CoNLL-2012, however, it contains documents from a different domain. 
CoNLL-2012 contains the newswire, broadcast news, broadcast conversation, telephone conversation, magazine, weblogs, and Bible genres while the annotated documents in WikiCoref are selected from Wikipedia.  


%Based on the results of Table~\ref{conll-2012-min-max-evaluations} and ~\ref{tab:gold_min_span}: (1) the use of minimum spans reduces the gap between the performance on gold vs.\ system mentions by about two percent, (2) the use of minimum instead of maximum spans results in a different ordering for some of the coreference resolvers, and (3) when gold mentions are used, there are no boundary detection errors, and consequently the results using \mina are the same as those of using maximum spans.\footnote{Due to recognizing the same head for distinct overlapping mentions, the scores using the head of gold mentions are not the same as using their maximum span, which in turn indicates \mina is suited better for detecting minimum spans compared to head words.}


%

\subsection{Results}
Table~\ref{tab:state_of_the_art} shows the maximum vs.\ minimum span evaluations of several recent coreference resolvers on the CoNLL-2012 test set and the WikiCoref dataset.
The examined coreference resolvers are as follows: the Stanford rule-based system \cite{leeheeyoung13},
the coreference resolver of \newcite{penghaoruo15},
the ranking model of \texttt{cort} \cite{martschat15c}, the ranking and reinforcement learning models of \texttt{deep-coref} \cite{clarkkevin16a,clarkkevin16b}, 
the single and ensemble models of \newcite{leekenton17}, and the current state-of-the-art system by \newcite{N18-2108}.
%\footnote{We did not have access to \newcite{penghaoruo15} and cort results on WikiCoref.}
%There are 92 annotated singletons in the WikiCoref dataset that are removed from the evaluation.

%i.e.\ mention maximum boundary detection errors that do not 
%affect the overall understanding of the text's entities can drop the performance up to two percent.
We make the following observations based on the results of Table~\ref{tab:state_of_the_art}:

\paragraph{Using minimum spans in coreference evaluation strongly affects the comparisons in the cross-dataset setting.}
The results on the WikiCoref dataset show that mention boundary detection errors specifically affect coreference scores in cross-dataset evaluations.
The ranking of systems is very different by using maximum vs. minimum spans.
The reinforcement learning model of \texttt{deep-coref}, i.e.,\ \texttt{deep-coref RL}, has the most significant difference when it is evaluated based on maximum vs.\ minimum spans (about 4 points).
%\texttt{deep-coref RL} and \texttt{deep-coref ranking} use different versions of the Stanford mention detection.
%While the newer variation that is used in \texttt{deep-coref RL} improves the results on CoNLL \cite{clarkkevin16b},
%it affects the mention detection in WikiCoref negatively.\footnote{For instance, in some cases \texttt{deep-coref RL} mention detection also includes the surrounding quotation marks or the following commas in the mention boundary, while it is not the case for gold mention boundaries.}
The ensemble model of \texttt{e2e-coref}, on the other hand, has the least difference between maximum and minimum span scores (1.4 points), which indicates it better recognizes maximum span boundaries in out-of-domain data.

\paragraph{Using minimum spans in coreference evaluation reduces the gap between the performance on gold vs.\ system mentions.}
It is shown that there is a large gap between the performance of a coreference resolver on gold vs.\ system mentions, see e.g., \newcite{penghaoruo15}.
The use of minimum spans in coreference evaluation reduces this gap by about two points. The comparison of the results of different systems on gold and system mentions using both maximum and minimum spans are included in Appendix~\ref{sec:appendix}.

\paragraph{Evaluation based on minimum spans reduces the differences that are merely due to better maximum boundary detection.}
The coreference resolver of \newcite{penghaoruo15} 
has the smallest difference between its maximum and minimum span evaluation scores.
This result indicates the superiority of \newcite{penghaoruo15}'s mention boundary detection method compared to other approaches.\footnote{It has a separate classifier for detecting maximum boundaries based on mention heads.}
Based on maximum spans, \newcite{penghaoruo15} performs on-par with \texttt{cort} while \texttt{cort} outperforms it by about one percent when they are evaluated based on minimum spans.
Therefore, the use of minimum spans in coreference evaluation decreases the effect of mention boundary detection errors in coreference evaluation and results in fairer comparisons.


%As we can see, based on maximum spans, the performance of the reinforcement learning approach of \newcite{clarkkevin16b} is about one percent worse than the rule-based system.
%However, if we use minimum spans, it outperforms the rule-based system.

%The results of ``max span'' vs.\ ``min span-gold'' show that 
%parsing errors or complexities affect the performance about two percent in maximum span evaluation,
%while based on ``min span-gold'' vs.\ ``min span-sys'' results, this effect is only about 0.2 percent in minimum span evaluation.
%The ``min span-gold'' vs.\ ``min span-sys'' results also show that the availability of gold parse trees is not essential for our minimum span extraction algorithm.
%As a result, MINA is applicable to corpora that do not contain gold parse information.
%For minimum span evaluations, we also report the evaluation of the CoNLL test data compared to itself,
%i.e.\ ``gold'' in Table~\ref{tab:state_of_the_art_min_gold_sys}.
%When a system is compared to itself, all evaluation scores should be 100\%.
%However, the performance drops because of
%few overlapping mentions that belong to two different entities 
%while the algorithm detects the same minimum span for them.
%Therefore, in minimum span evaluations one minimum span is assigned to two different entities.
%This problem occurs only in a very few examples and because
%of errors in parse trees and few coreference annotation errors,
%e.g.\ ``[[Attorney Richard Jackson]$_1$ of Dallas]$_2$ says a judgment''.
%

%Table~\ref{tab:wikicoref_max_min_span} shows the use of minimum spans in the WikiCoref dataset \cite{ghaddar16b} that does not contain gold parse information.
%This dataset is used for out-of-domain evaluation of systems that are trained on CoNLL \cite{ghaddar16a,moosavi17b}.
%\footnote{By using the option \texttt{remove\_singletons} in the \texttt{scorer.py} command}.




 

==> mina_acl2019/eval.tex <==
\section{Evaluating MINA Spans}
In order to analyze the detected \mina spans, we evaluate the following two properties: 
\squishlist
\item Length of \mina spans: since we retrieve \mina spans from the corresponding parse tree of the mentions, \mina spans are always a subset of their corresponding maximum span words. 
However, on average, the length of minimum spans (number of containing words) should be smaller than that of maximum spans.
\item Compatibility of automatically extracted minimum spans with those that are manually annotated by experts: we evaluate \mina spans against manually annotated minimum spans, called \texttt{MIN}, in the MUC and ARRAU corpora to examine whether the reduced spans still contain words of the mention that were deemed important by experts. 
%\item Minimum span of distinct mentions: if we have two distinct maximum spans, their corresponding minimum span should also be different. This property is of particular importance for overlapping mentions. 
%The minimum span of two different overlapping maximum spans should not be equal. As an example, the minimum span of the mention "John and Mary" should be different from those of ``John'' and ``Mary'', because they all refer to different entities.
\squishend

For the experiments of this section, we use the MUC-6, MUC-7, ARRAU, and CoNLL-2012 corpora, from which MUC and ARRAU contain manually annotated minimum spans.
We use the Stanford neural constituency parser \cite{socher13parse} for getting system parse trees, unless otherwise stated.
For the ARRAU corpus, we use mentions of the training split of the RST Discourse Treebank subpart.

As a baseline, we also evaluate the syntactic head of mentions, based on Collins' rules, as the minimum span.\footnote{We use the implementation of the head-finding rules that is available at \url{https://github.com/smartschat/cort/}.}


%\paragraph{Baseline}
%As an alternative to \mina spans, we can consider the syntactic head of mentions as their minimum span. 
%We use Colins' head finder rules \cite{collins2003head} for determining mention heads.
%Mention heads haven been used by \newcite{penghaoruo15} as an alternative for maximum spans in coreference evaluation, driven by a similar motivation as that of this paper, i.e.\ reducing the effect of mention boundary detection in coreference evaluation. 


\paragraph{How does the length of evaluated spans change by using MINA?}
Table~\ref{tab:min-span-head-len} shows the average length of maximum spans vs. that of \mina spans on the training splits of the MUC-6, MUC-7 and ARRAU corpora as well as the development set of the CoNLL-2012 dataset. 
For the CoNLL-2012 dataset, we use the provided gold parse information.
We parse the MUC and ARRAU datasets,
% with the Stanford neural constituency parser \cite{socher13parse},
since the gold parse information is not available for these datasets.

Based on Collins' head finder rules, the detected head always includes one word.
%The ratio of mentions for which the length of \mina minimum span is different (i.e.\ smaller) from that of the maximum span is 42\%.

\begin{table}[!htb]
    \begin{center}
        \resizebox{\columnwidth}{!}{%

    \begin{tabular}{l|llll}
		& MUC-6 & MUC-7 & ARRAU & CoNLL\\ \hline
		maximum span & $5.2$ & $5.3$ & $3.8$ & $2.4$\\ \hline
		\mina span & $2.6$ & $2.7$ & $2.0$ & $1.6$\\ 
    \end{tabular}
}
    \end{center}
    \caption{The average length of \mina spans compared to that of maximum spans in the MUC, ARRAU, and CoNLL-2012 datasets.}
    \label{tab:min-span-head-len}
\end{table}

Figure~\ref{fig:span_length} shows the number of mentions with the length of one, two, three, and $\geq$4 based on both maximum and \mina spans on the CoNLL-2012 development set. 
The length of the maximum span of around $14\%$ of mentions is longer than three, while this ratio is only $4\%$ for \mina minimum spans.  
Mentions with long \mina spans include appositions or conjunctions, e.g.,\ the \mina span in Figure~\ref{fig:mina-example4}.

\begin{figure}
    \centering
\resizebox{0.92\columnwidth}{!}{%
\begin{tikzpicture}
\begin{axis}[
    ybar,
    enlargelimits=0.15, legend pos=north,
    legend style={at={(0.6,0.9)},anchor=north east,%at={(0.5,-0.1)},
      anchor=north,legend columns=-1},
    xlabel={Span length},   ylabel={Count},  ylabel near ticks,
    symbolic x coords={1,2,3,more},
    xtick=data, ybar=4pt, width=\columnwidth,
    %nodes near coords,
    nodes near coords align={vertical},
    ]
\addplot [fill=blue] coordinates {(1,11125) (2,3820) (3,1499) (more,2712)};
\addplot coordinates {(1,11684) (2,4866) (3,1828) (more,778)};
\legend{max-span,min-span}
\end{axis}
\end{tikzpicture}
}
\caption{Span length based on maximum vs. \mina's minimum spans on the CoNLL-2012 development set.}
\label{fig:span_length}
\end{figure}


%\{``the company'', ``William G. Moore Jr.'', ``Robert W. Reedy'', ``five defendants''\} is \mina span for the mention ``the company, former chief executive officer William G. Moore Jr., former vice president Robert W. Reedy and five defendants who weren't part of the company''.


%" 200 hectares of land at the foot of Lantau Island that was obtained following the largest land reclamation project in recent years" -> 200 hectares

%This result shows that \mina considerably reduces the length of evaluated span in coreference evaluation.
%As a result, there is a smaller chance that parsing errors in mention boundary detection would affect coreference evaluation.


\paragraph{Does MINA correlate with MIN?}
%The results of Figure~\ref{fig:span_length} shows that the length of \mina minimum spans is smaller than those of maximum spans.
%In order to validate whether these shortened spans still contain the most important part of the mentions, 
We evaluate \mina minimum spans against manually annotated minimum spans in the MUC and ARRAU corpora.
The manually annotated minimum span in these corpora is referred to as \texttt{MIN}.
%As in the above experiments, we parse these corpora with the Stanford neural parser \newcite{socher13parse}.

Table~\ref{tab:min-span-head-min} shows the ratio of minimum spans that contain the corresponding \texttt{MIN} when the minimum span is extracted by \mina and the head finding rules. 
As we can see, \mina contains \texttt{MIN} in the majority of the mentions, and therefore, it is compatible with what experts would consider as the most important part of the mentions.

\begin{table}[!htb]
    \begin{center}
    \begin{tabular}{l|lll}
		& MUC-6 & MUC-7 & ARRAU\\ \hline
		\mina & $96.2$ & $93.1$ & $98.3$ \\ \hline
		head & $94.0$ & $91.1$ & $93.9$ \\
    \end{tabular}

    \end{center}
    \caption{Ratio of detected \mina and head words which contain the corresponding \texttt{MIN} annotations in the MUC and ARRAU corpora. The same parse information is used for detecting both \mina and head words. 
    Datasets are parsed using the Stanford neural parser.
    }
    \label{tab:min-span-head-min}
\end{table}


Figure~\ref{fig:arrau-mina-vs-head} shows an example from ARRAU in which \mina contains \texttt{MIN} but the head does not.

\begin{figure}[!htb]
\centering
 \resizebox{0.9\columnwidth}{!}{\Tree[.NP \textbf{many big} [.UCP oil, chemical and airline ] \textbf{companies} ]}
\caption{System parse tree of a mention from ARRAU. \mina spans are boldfaced. ``many'' and ``companies'' are the corresponding \texttt{MIN} and head, respectively. \label{fig:arrau-mina-vs-head}}
\end{figure}

\mina and \texttt{MIN} inconsistencies, i.e.,\ cases in which \mina does not contain \texttt{MIN}, are mainly due to parsing errors. 
Figure~\ref{fig:muc6-parsing-error} and Figure~\ref{fig:arrau-parsing-error} show two examples from the MUC and ARRAU datasets in which \mina selects an incorrect minimum span because of an incorrect parse tree.  

%For instance, for the mention ``a very tough job'' (Figure~\ref{fig:muc7-example1}) from MUC-7, \mina selects ``a job'' as the minimum span while ``job'' is only annotated as MIN.

%\begin{figure}[!htb]
%\centering
% \resizebox{0.4\columnwidth}{!}{\Tree [.NP \textbf{a} [.ADJP very tough ] \textbf{job} ]}
%\caption{The system parse tree of the mention ``a very tough job'' from MUC-7.\label{fig:muc7-example1}}
%\end{figure}

\begin{figure}[!htb]
\centering
 \resizebox{0.8\columnwidth}{!}{\Tree [.S [.NP \textbf{American} ][.VP 's [.NP [.QP \text{more than 10000} ] \text{flight attendants} ]]]}
\caption{The system parse tree of a mention from MUC-6. \mina spans are boldfaced (``American''). ``attendants'' is the annotated MIN.\label{fig:muc6-parsing-error}}
\end{figure}

\begin{figure}[!htb]
\centering
 \resizebox{0.65\columnwidth}{!}{\Tree [.NP [.NP \textbf{the first} ][.SBAR [.WHNP [.NP time ][.PP since [.NP \text{January 1987} ]]]]]}
\caption{The system parse tree of a mention from ARRAU. \mina spans are boldfaced (``the first''). ``time'' is the annotated MIN.\label{fig:arrau-parsing-error}}
\end{figure}

Figure~\ref{fig:arrau-true-mismatch} shows two sample mismatch examples between \mina and \texttt{MIN} from the ARRAU dataset, in which the mismatch is not due to parsing errors.

\begin{figure}[!htb]
\centering
 \resizebox{\columnwidth}{!}{\Tree [.NP [.QP \textbf{268 million} ][.PP in [.NP [.NP cash ] and [.NP marketable securities ]]]] \Tree[.NP [.NP [.QP \textbf{329 million} ]][.PP in [.NP cash ]]]}
\caption{The system parse trees of two mentions from ARRAU. \mina spans are boldfaced. ``securities'' and ``cash'' are annotated as \texttt{MIN} for the left and right mentions, respectively.  \label{fig:arrau-true-mismatch}}
\end{figure}

In order to investigate the effect of using a different parser,
we perform the experiment of Table~\ref{tab:min-span-head-min} using the Stanford English PCFG parser \cite{klein03b}.
The results are reported in Table~\ref{tab:min-span-head-min-pcfg}.
As we see, the use of a better parser, i.e.,\ the Stanford neural parser, makes \mina spans, as well as detected heads, more consistent compared to \texttt{MIN} spans.

\begin{table}[!htb]
    \begin{center}
    \begin{tabular}{l|rrr}
		& MUC-6 & MUC-7 & ARRAU\\ \hline
		\mina & $95.6$ & $92.4$ & $98.1$ \\ \hline
		head & $92.9$ & $90.0$  & $93.4$ \\
    \end{tabular}

    \end{center}
    \caption{Ratio of the detected \mina and head words that contain their corresponding \texttt{MIN} annotations in MUC and ARRAU. \mina and head words are detected using the parse trees of the Stanford PCFG parser.}
    \label{tab:min-span-head-min-pcfg}
\end{table}






%The mention ``the new Chief of Naval Operations'' from MUC-7 is an example of mismatches for which ``Chief of Naval Operations'' and ``the new Chief'' are the corresponding \mina and MIN spans, respectively.
%As long as we use the same algorithm to extract minimum spans for both gold and system mentions, such differences will not affect the evaluation.


%\begin{figure}
%\centering
% \resizebox{\columnwidth}{!}{\Tree [.QP \textbf{\$ 500 million} ] \Tree[.PP in [.NP [.NP debt ] [.VP owed [.PP to [.NP the parent ]]]]]}
%\caption{The system parse tree of the mention ``\$ 500 million in debt owed to the parent'' from ARRAU, in which \mina and MIN are ``\$ 500 million'' and ``parent'', respectively.  \label{fig:arrau-true-mismatch2}}
%\end{figure}


%For instance, for our example, ``Corp.'' and ``presence'' would only be selected as minimum spans in manual annotations.
%However, in the majority of the examined mentions, the extracted minimum spans do include and therefore are compatible with the manually annotated ones. 


%\paragraph{Does MINA detects different minimum spans for distinct overlapping mentions?}
%As mentioned above, the detected minimum span for two distinct overlapping mention should be different. 
%For instance in ``securities'' 
%For this analysis, we examine all the annotated overlapping mentions in the CoNLL-2012 development set.

In addition to the above two properties, i.e.\ the length of minimum spans and their consistency with \texttt{MIN} annotations, we also check that \mina returns \emph{different minimum spans for distinct overlapping mentions}.


As an example, the minimum span of the mention ``John and Mary'' should be different from those of ``John'' and ``Mary'', because they all refer to different entities. In this regard, we examine all overlapping coreferent mentions in the CoNLL-2012 English development set, from which none of the overlapping mentions has the same \mina span. However, this is not the case for heads.

==> mina_acl2019/exmp.tex <==
\section{Boundary Mismatch Example}
Example~\ref{example}, and its corresponding gold and system parse trees in Figure~\ref{extensive_presence_gold_parse} and Figure~\ref{extensive_presence_sys_parse}, respectively, show a sample boundary mismatch from the CoNLL-2012 development set.
%respectively.\footnote{We take the example and its corresponding gold and system parse trees from the CoNLL-2012 development set.}
Based on the gold parse tree (Figure~\ref{extensive_presence_gold_parse}),
``an extensive presence'' is the maximum span of the first coreferring mention in Example~\ref{example}.
However, the corresponding maximum boundary for this same mention is ``an extensive presence, of course in this country'' based on the system parse tree (Figure~\ref{extensive_presence_sys_parse}).

\begin{example}
 This News Corp. has [an extensive presence]$_{1}$, of course in this country.
 [That presence]$_{(1)}$ may be expanding soon.
 \label{example}
\end{example}

\begin{figure}[!htb]
\centering
 \resizebox{0.98\linewidth}{!}{\Tree [.S [.NP \text{This News Corp.} ] [.VP has [.NP [.NP \text{an extensive presence} ]] , [.PP of [.NP course ]][.PP in [.NP \text{this country} ]]]]}
\caption{Gold parse tree of Example~\ref{example}.\label{extensive_presence_gold_parse}}
\end{figure}
\begin{figure}[!htb]
\centering
 \resizebox{0.9\linewidth}{!}{\Tree [.S [.NP \text{This News Corp.} ][.VP has [.NP [.NP [.NP \text{an extensive presence} ] , [.PP of [.NP course ]]] [.PP in [.NP \text{this country} ]]]]]}
\caption{System parse tree of  Example~\ref{example}.\label{extensive_presence_sys_parse}}
\end{figure}

A system that uses the system parse tree for mention detection
links ``that presence'' to ``an extensive presence, of course in this country''
and gets penalized based on recall and precision. 
This penalty is the same as that of a system that links ``that presence'' to ``this News Corp.''.
Recall drops because of not recognizing ``an extensive presence''
and precision drops because of detecting a spurious mention.
%As a result, evaluation based on maximum spans explicitly penalizes resolvers because of parsing variations. 


==> mina_acl2019/how.tex <==
\section{How to Determine Minimum Spans?}
\label{sect:how}
We process the constituency-based parse trees of mentions, i.e.,\ the parse sub-tree of their corresponding maximum span, in a breadth-first manner to determine minimum spans.
Algorithm~\ref{min-span-algo} outlines the minimum span extraction process.
In this algorithm, \texttt{root} is the root of the mention's parse tree, \texttt{tags} is the set of acceptable syntactic tags for extracting minimum spans, \texttt{min-depth} is the depth of the minimum span nodes in the parse tree, and \texttt{min-spans} is the output of the algorithm that corresponds to the set of mention words that belong to the minimum span.
\texttt{min-depth} is initially set to $\infty$, and \texttt{tags} and \texttt{min-spans} are empty.

\begin{algorithm}[!htb]
\footnotesize
\SetAlgoLined
\DontPrintSemicolon 
%\SetAlFnt{\small}
       %\SetKwInOut{Input}{roo}
       % \SetKwInOut{Output}{output}
       % \Input{root: the root of the mention parse tree}
       % \Output{min-spans: the set of mention words that are included in the minimum span}
\SetKwFunction{algo}{MINA}
\SetKwProg{myalg}{Algorithm}{}{}
  \myalg{\algo{root}}{
  
   min-depth = \infty \;
     
   \If{tags=$\emptyset$}{
       \If{\text{root is an NP}}{
             \text{tags= \{NP acceptable tags\}}}
          \ElseIf{\text{root is a VP}} {
             \text{tags=\{VP acceptable tags\}}\;
          }
       }
   \text{Process $root$ in a breadth-first manner} \;
   \For{each processed node $n$ \text{ } }{
   \If{$n$.tag \not\in tags \text{ }}{
       \text{skip processing $n$'s children} \;
   }
   \ElseIf{$n$ \text{is an acceptable terminal node} \And $n$.depth\leq $min-depth$ \text{ }}{
      min-spans.add(n)\;
	  min-depth = n.depth \;
    }
   }
   
   
  }
  
\caption{Extraction of minimum spans.}
%Initially, \texttt{root} is the root of the parse tree of the mention maximum span. \texttt{tags} would be set to \{NP, NML, QP, NX\} for the tree of a noun phrase and \{VP\} for that of a verb phrase. The mention words that belong to the minimum span are collected in \texttt{min-spans}.}
\label{min-span-algo}
\end{algorithm}


The set of acceptable terminal nodes in a parse tree are those that include at least one word other than a determiner\footnote{A word with the ``DT'' POS tag.} or a conjunction\footnote{A word with the ``CC'' POS tag.}.
We do not further split terminal nodes, e.g., an acceptable terminal node may contain both a determiner as well as a noun.
For extracting the minimum span of a noun phrase, the set of acceptable syntactic tags is \{``NP'' (noun phrase), ``NML'' (nominal modifier), ``QP'' (quantifier phrase used within NP), ``NX'' (used within certain complex NPs)\}. For verb phrases, ``VP'' is the only acceptable tag.

\mina processes the parse tree in a breadth-first manner.
It skips processing sub-trees that are rooted by a node whose syntactic tag is not acceptable, e.g., ``PP''.
For the rest of the nodes, it extracts all acceptable terminal nodes that have the shortest distance to \texttt{root} as minimum spans.

%If \texttt{root} contains an acceptable terminal child, then the minimum span would be the set of all acceptable terminal children.
%For instance, the root of the parse tree in Figure~\ref{fig:mina-example2} includes two acceptable terminal children, i.e.,\ ``new'' and ``zone'', which would be selected by \mina as the minimum spans.  

%If \texttt{root} does not have any acceptable terminal children, \mina recursively processes all of its non-terminal children that have acceptable syntactic tags.

For instance, in Figure~\ref{fig:mina-example5}, the root node is an NP and \texttt{tag} would be set to NP's acceptable tags. Therefore, among the children of the root, \mina would only process the child with an NP tag (the left child) and skip the one with the PP tag.  

If the final minimum span is empty, e.g.,\ if due to parsing errors the syntactic tag of none of the tree nodes is among the acceptable tags, we fall back to using the maximum span.\footnote{If we use gold parse trees, 
this happens for 14 mentions in the CoNLL-2012 development set
from which ten are one-word mentions,
e.g.,\ ``ours'' is detected as ``ADJP''.}

%Given a minimum span and the parse tree that it has been extracted from, 
%we can reconstruct the maximum span by finding the common NP (or VP) parent that includes all the corresponding terminal nodes of the minimum span. 


%If we instead use system parse trees,
%above numbers are 60 and 51, respectively. 
\paragraph{MINA extraction examples.}
Figures~\ref{fig:mina-example5}-\ref{fig:mina-example4} show the \mina minimum spans of various noun phrases with different internal structures. The corresponding \mina spans of the parse trees are boldfaced. 
%\begin{figure}[!htb]
%\centering
% \resizebox{0.23\columnwidth}{!}{\Tree [.NP \textbf{January 3} ]}
%\caption{\mina span in an NP with acceptable terminal nodes. \mina spans are boldfaced.\label{fig:mina-example0}}
%\end{figure}

%\begin{figure}[!htb]
%\centering
% \resizebox{0.7\columnwidth}{!}{\Tree [.NP [.NP \textbf{that statement} ] [.SBAR [.WHNP that ][.S [.NP Jordan ][.VP made ]]]]}
%\caption{\mina span in an NP with the grammar form ``NP $->$ NP SBAR''. \mina spans are boldfaced.\label{fig:mina-example1}}
%\end{figure}

\begin{figure}[!htb]
\centering
 \resizebox{0.8\columnwidth}{!}{\Tree [.NP [.NP \textbf{a copy} ][.PP of [.NP \text{the statement} ]][.PP from [.NP \text{the newspapers} ]]]}
 %\Tree[.NP [.NP \textbf{the working meeting} ][.PP of [.NP \text{the program} ]]]
 % and ``NP $->$ NP PP'' in the left and right sub-tree, respectively
\caption{\mina span in an NP with the grammar form ``NP $->$ NP PP PP''. \mina span is boldfaced.\label{fig:mina-example5}}
\end{figure}

\begin{figure}[!htb]
\centering
 \resizebox{0.95\columnwidth}{!}{\Tree [.NP [.NP Shantou's ] \textbf{new} [.NML [.NML [.NML high level ] technology ] development ] \textbf{zone} ]}
\caption{\mina spans in an NP with a nested structure.\label{fig:mina-example2}}
\end{figure}

\begin{figure}[!htb]
\centering
 \resizebox{0.95\columnwidth}{!}{\Tree [.NP [.NP [.NP \textbf{a man} ][.VP named [.NP Cornelius ]]][.NP [.NP \textbf{a Roman army officer} ][.PP in [.NP \text{the Italian unit} ]]]]}
\caption{\mina spans in an appositive noun phrase.\label{fig:mina-example3}}
\end{figure}

\begin{figure}[!htb]
\centering
 \resizebox{0.95\columnwidth}{!}{\Tree [.NP [.NP \textbf{Joran Van Der Sloot} ][.NP \textbf{Deepak Kalpoe} ] and [.NP \textbf{Satish Kalpoe} ]]}
\caption{\mina spans in an NP with conjunction. Boldfaced minimum spans belong to a single mention.\label{fig:mina-example4}}
\end{figure}


%For instance, consider the subtree of Figure~\ref{extensive_presence_sys_parse} that starts with the root NP node of ``an extensive presence, of course in this country''.
%For this subtree, ``valid-tags'' is initialized to \{NP, NML, QP, NX\}.
%The only path of this tree in which all nodes have valid tags
%is the one that ends to the terminal nodes ``an extensive presence'',
%which in turn is selected as the minimum span.
\paragraph{Using MINA for coreference evaluation.} 
%We incorporate the \mina algorithm in a coreference evaluation package with all standard evaluation metrics.
%This package provides coreference evaluation scores based on maximum spans (the default evaluation setting) and \mina spans. Besides, we also provide an evaluation option for determining minimum spans based on Collins' syntactic heads instead of the \mina algorithm.
%\footnote{This package will be made publicly available upon publication.}
For each coreference evaluation, we have a key file, including gold coreference annotations, and a system file, including predicted coreference outputs.
For coreference evaluation using minimum spans, we use the provided parse trees in the key file.\footnote{If the key file does not include parse information, we parse it with the Stanford parser.} 
Therefore, the minimum spans of both gold mentions and system mentions are determined based on the same parse tree.
We then use minimum spans instead of maximum spans in all scoring metrics, i.e.,\ a gold and a system mention are considered equivalent if they have the same minimum span.

The corresponding sub-trees of the discussed gold and system mentions of Example~\ref{example}, based on the gold parse tree in Figure~\ref{extensive_presence_gold_parse}, are shown in Figure~\ref{fig:example-1-min-spans}.\footnote{If the boundary of a mention is not recognized as a single phrase in the parse tree, as it is the case for the system mention, we add a dummy root (``X'' in the right subtree of Figure~\ref{fig:example-1-min-spans}) to include the whole span into a single phrase.}
The \mina span of both of these two trees is ``an extensive presence''. Therefore, the gold coreference chain \{``an extensive presence'', ``that presence''\} and the system coreference chain \{``an extensive presence, of course in this country'', ``that presence''\} are equivalent if they are evaluated based on minimum spans.

\begin{figure}[!htb]
\centering
 \resizebox{0.95\columnwidth}{!}{\Tree [.NP [.NP \textbf{an extensive presence} ]] \Tree[.X [.NP [.NP \textbf{an extensive presence} ]] , [.PP of [.NP course ]][.PP in [.NP \text{this country} ]]]}
\caption{Mention trees of Example~\ref{example}. The left and right sub-trees represent the boundaries of gold and system mentions, respectively. \label{fig:example-1-min-spans}}
\end{figure}

%If gold parse trees are provided in the examined corpus, we extract minimum spans of both gold and system mentions
%based on the gold parse trees.
%If the given corpus does not include the syntactic parse information, we automatically parse it using the 
%Stanford English PCFG parser \cite{klein03b}\footnote{More recent parsers can also be used at the expense of increased parsing time.}. 
%Please note that in this evaluation setting, the assumption is that the coreference resolvers are all trained to resolve and detect maximum spans, as it is the case for almost all existing coreference resolvers.


==> mina_acl2019/intro.tex <==
\section{Introduction}
\label{sect:intro}
Coreference resolution is the task of finding different expressions that refer to the same real-world entity. Each referring expression is called a mention.
The common approach to annotate coreferring mentions is to specify the largest span of each mention.
The problem with using maximum spans in coreference evaluation is that a single mention may have different maximum boundaries based on gold vs. automatically detected syntactic structures.
%For instance, a single mention may have two different maximum boundaries based on gold vs.\ automatically detected syntactic structures.
%, from which gold syntax is used in gold coreference annotations while coreference resolvers automatically detect maximum mention boundaries without using gold information.
For instance, variations in prepositional phrase attachment, which is a known challenge in syntactic parsing, will lead to different maximum boundaries for a single mention.
%Many such mismatches between maximum boundaries that are extracted based on gold vs.\ system trees
%are due to .

In order to decouple coreference evaluation from maximum boundary detection complexities,
smaller corpora like MUC \cite{hirschman97}, ACE \cite{ace2002data}, and ARRAU \cite{arrau}
explicitly annotate the minimum span as well as the maximum logical span of each mention.
The annotated minimum spans indicate the minimum strings that a coreference resolver must identify for the corresponding mentions. 
%If a coreference resolver identifies the minimum span instead of the corresponding maximum boundary,
%it will receive full credit.
This solution comes with an additional annotation cost.
As a result, the annotation of minimum spans has been discarded in larger corpora like CoNLL-2012 \cite{2012-ontonotes}.

In this paper, we propose \mina, a MINimum span extraction Algorithm that
automatically determines minimum spans from constituency-based parse trees.
Based on our analyses,
\mina spans are compatible with those that are manually annotated by experts.
By using \mina, we can benefit from minimum span evaluation
for all corpora without introducing additional annotation costs.

While the use of \mina spans already benefits in-domain evaluation, by reducing the gap between the performance on gold vs.\ system mentions, it has a more significant impact on cross-dataset evaluation, in which detected maximum mention boundaries are noisier due to domain shift.

Cross-dataset coreference evaluation is used to assess the generalization of coreference resolvers \cite{moosavi-strube-2017-lexical,moosavi-strube-2018-using}. 
Coreference resolution is a mid-step for text understanding in downstream tasks, e.g., question answering, text summarization, and information retrieval. 
Therefore, generalization is an important property for coreference resolvers because downstream datasets are not necessarily from the same domain as those of coreference-annotated corpora. 

When coreference resolvers are applied to a new domain, detected maximum boundaries become noisier, e.g., gold and system mentions differ by the inclusion or exclusion of surrounding commas or quotation marks.
Such noisy boundaries directly affect the coreference evaluation scores based on maximum spans.
The use of minimum spans reduces the impact of such noises in coreference evaluation and results in more reliable comparisons between different coreference resolvers.

%A coreference resolver can benefit a downstream application by determining all pieces of the context that are related to the entity\footnote{E.g., for answering a question about that entity}, or by disambiguation of pronouns\footnote{E.g., to correctly translate pronouns in languages with grammatical gender}.
%The generalization of coreference resolvers is determined by cross-dataset evaluations, e.g., \cite{P17-2003}.


%Incorporating minimum spans in coreference evaluation has the following advantages:
%\begin{itemize}
%\item It reduces the gap between the performance on gold vs.\ system mentions by about two percent.
%\item It decreases differences between different coreference resolvers that are merely due to better maximum boundary detection and not better resolution of coreference relations.
%\item It has a significant impact on cross-dataset coreference evaluation, in which the detection of maximum boundaries is not as accurate as in in-domain evaluations. 
%\end{itemize}

%Besides, compared to manually annotated minimum spans, the use of automatically annotated minimum spans can better handle boundary mismatches as explained in \autoref{sect:rel}.

%We will provide our coreference evaluation package that reports all standard coreference evaluation metrics using both maximum and \mina spans upon the publication.
%and will be made publicly available upon publication.


==> mina_acl2019/name.tex <==
\begin{table*}[!htb]
    \begin{center}
        %\resizebox{\columnwidth}{!}{%
    \begin{tabular}{@{}l|l|l||l|l||l|l||l|l@{}}
		\multicolumn{1}{c}{} & \multicolumn{2}{c}{maximum span} & \multicolumn{2}{c}{MINA span} & \multicolumn{2}{c}{head} &  \multicolumn{2}{c}{gold mentions}\\
     & CoNLL & LEA & CoNLL & LEA & CoNLL & LEA & CoNLL & LEA\\ \hline
    \hline
    fernandes &$60.6$  & $53.3$ (1) & $61.80$ & $54.71$ (1) & $57.03$  & $63.91$ & $69.36$ & $56.07$ \\
    martschat & $57.7$ & $50.0$ (2) & $59.18$ & $51.93$ (2) & $61.03$  & $53.89$ & -& -\\
    bjorkelund&  $57.4$  & $50.0$ (3)& $58.24$ & $51.05$ (3) & $60.68$ & $53.57$ & $67.97$ & $61.06$\\
    chang & $56.1$ & $48.5$ (4)& $57.58$ & $50.38$ (4) & $59.62$ & $52.46$ & $77.23$ & $67.87$\\
    chen& $54.5$ & $46.2$ (6)& $55.82$  & $48.25$ (5) & $58.22$ & $50.43$ & $71.34$ & $63.95$\\
    chunyuang& $54.2$ & $45.8$ (7) & $55.18$ & $47.56$ (7) & $57.88$ & $50.16$ & - & -\\
    shou & $53.0$ & $44.0$ (9) & $54.03$ & $45.68$ (8) & $56.54$ & $48.09$ & -&-\\
    yuan &$52.9$  & $44.8$ (8) & $54.74$ & $46.91$ (8) & $56.68$ & $48.87$ & $70.45$ & $63.45$\\
    xu &$52.6$ & $46.8$ (5) & $53.76$  & $48.29$ (5) & $55.21$ & $49.97$ & $60.96$ & $56.88$\\
    uryupina &$50.0$ & $41.2$ (11) & $50.93$ & $42.24$ (10) & $52.45$ & $43.72$ & - &-\\
    songyang & $49.4$ & $41.26$ (10) & $50.92$ & $43.21$ (10) & $52.86$ & $45.34$ & -&-\\
    %zhekova & $40.45$  & $29.98$ (12) & $42.26$ & $31.90$ (13) \\
    %xinxin & $38.63$ & $29.22$ (12) & $41.39$ & $32.05$ (12)\\
    %li &$36.11$ & $27.32$ (14) & $36.40$ & $27.59$ (14)\\
    %stamborg & \\
    \end{tabular}
    %}
    \end{center}
    \caption{CoNLL-2012 shared task systems evaluations}
    \label{conll-2012-min-max-evaluations}
\end{table*}

Compared to manual annotations, automatically extracted minimum spans have the following advantages:
%\squishlist
\begin{enumerate}
\item By using \mina, we can benefit from minimum span evaluation
for all corpora without introducing additional annotation costs, 
while manually annotated minimum spans are only applicable in their own corpora. 
%MINA is applicable for all English coreference corpora while 
%we can only benefit from manually annotated minimum spans in their own corpora.
As we show, MINA minimum spans are compatible with the annotated ones.
%
\item According to the MUC task definition\footnote{\url{http://www-nlpir.nist.gov/related_projects/muc/proceedings/co_task.html}},
the use of minimum spans in coreference evaluation is as follows:\footnote{This use of minimum spans is also followed by the ARRAU dataset}
Assume $m_{max}$ and $m_{min}$ are annotated maximum and minimum spans for the mention $m$.
The system mention $\hat{m}$ is equivalent to $m$ if it includes $m_{min}$ and it does not 
include any token beyond those that are included in $m_{max}$.
This way of using minimum spans does not handle inconsistencies in gold vs. system mention boundaries 
in which system boundaries are larger than their corresponding gold boundaries, 
as it is the case for the mention ``an extensive presence, of course in this country'' in Example~\ref{example}.
However, as we explain in Section~\ref{sect:how}, \mina extracts minimum spans for both gold and system mentions based on the same parse tree, and can handle system detected maximum spans that are either shorter or longer than theor corresponding gold maximum span.
%\squishend
\end{enumerate}

\begin{table*}[!htb]
    \begin{center}
        %\resizebox{\columnwidth}{!}{%
    \begin{tabular}{l|l|l||l|l||l|l}
		\multicolumn{1}{c}{} & \multicolumn{2}{c}{maximum span} & \multicolumn{2}{c}{MINA span} & \multicolumn{2}{c}{head} \\ %&  \multicolumn{2}{c}{gold mentions}
     & CoNLL & LEA & CoNLL & LEA & CoNLL & LEA\\ \hline
    \hline
    fernandes &$60.6$ (1) & $53.3$ (1) & $62.2$ & $55.1$ (1) & $63.9$ & $57.0$ (1)\\ %& $69.4$ & $56.1$ \\
    martschat & $57.7$ (2)& $50.0$ (2) & $59.7$ & $52.4$ (2) & $61.0$ & $53.9$ (2)\\ % & -& -\\
    bjorkelund&  $57.4$ (3) & $50.0$ (2)& $58.9$ & $51.6$ (3) & $60.7$ & $53.6$ (3)\\ %& $68.0$ & $61.1$\\
    chang & $56.1$ (4)& $48.5$ (4)& $58.0$ & $50.7$ (4)& $59.6$ & $52.5$ (4)\\ %& $77.2$ & $67.9$\\
    chen& $54.5$ (5)& $46.2$ (6)& $56.5$ & $48.6$ (5) & $58.2$ & $50.4$ (5)\\ %& $71.3$ & $63.9$\\
    chunyuang& $54.2$ (6)& $45.8$ (7) & $56.1$ & $48.1$ (7) & $57.9$ & $50.2$ (6)\\ %& - & -\\
    shou & $53.0$ (7)& $44.0$ (9) & $54.8$ & $46.1$ (9) & $56.5$ & $48.1$ (9)\\ %& -&-\\
    yuan &$52.9$  & $44.8$ (8) & $54.9$ & $47.0$ (8)& $56.7$ & $48.9$ (8)\\%& $70.4$ & $63.4$\\
    xu &$52.6$ & $46.8$ (5)  & $53.9$ & $48.4$ (6) & $55.2$ & $50.0$ (7)\\ % & $61.0$ & $56.9$\\
    uryupina &$50.0$ & $41.2$ (11) & $51.0$ & $42.3$ (11)& $52.4$ & $43.7$ (11)\\ % & - &-\\
    songyang & $49.4$ & $41.3$ (10) & $51.3$ & $43.5$ (10)& $52.9$ & $45.3$ (10)\\ %& -&-\\
    %zhekova & $40.45$  & $29.98$ (12) & $42.26$ & $31.90$ (13) \\
    %xinxin & $38.63$ & $29.22$ (12) & $41.39$ & $32.05$ (12)\\
    %li &$36.11$ & $27.32$ (14) & $36.40$ & $27.59$ (14)\\
    %stamborg & \\
    \end{tabular}
    %}
    \end{center}
    \caption{CoNLL-2012 shared task systems evaluations}
    \label{conll-2012-min-max-evaluations}
\end{table*}

==> mina_acl2019/rel.tex <==
\section{Background}
\label{sect:rel}
\mina is an attempt to decouple coreference evaluation from parsing errors
to some extent.
This motivation is the same as the one that resulted in the manual annotation of minimum spans in the 
MUC, ACE and ARRAU corpora.
According to the MUC task definition,\footnote{\url{http://www-nlpir.nist.gov/related_projects/muc/proceedings/co_task.html}}
the use of minimum spans in coreference evaluation is as follows:\footnote{The ARRAU dataset also follows this way of using minimum spans.}
Assume $m_{max}$ and $m_{min}$ are the annotated maximum and minimum spans for the mention $m$.
The system mention $\hat{m}$ is equivalent to $m$ if it includes $m_{min}$ and it does not 
include any tokens beyond those that are included in $m_{max}$.
This way of using minimum spans does not handle inconsistencies in gold vs. system mention boundaries 
in which system boundaries are larger than their corresponding gold boundaries, 
as it is the case for the mention ``an extensive presence, of course in this country'' in Example~\ref{example}.

Compared to manually annotated minimum spans:
\squishlist
\item \mina is applicable to any English coreference corpus.\footnote{We did not have the manually annotated minimum spans for coreference corpora of other languages in order to verify whether \mina is also applicable to them.} In contrast, manually annotated minimum spans can be only used in their own corpora.
\item For coreference evaluation, \mina extracts minimum spans for both gold and system mentions based on a single parse tree. Therefore, it can handle system-detected maximum spans that are either shorter or longer than their corresponding gold maximum span.  
\squishend

The coreference resolver of \newcite{penghaoruo15} is developed around the idea
that working with mention heads is more robust compared to working with maximum mention boundaries.
In this regard, they develop a system that resolves coreference relations based on mention heads.
The resolved mention heads are then expanded to full mention boundaries
using a separate classifier that is trained to do so. 
\newcite{penghaoruo15} also report the evaluation scores 
using both maximum mention boundaries and mention heads.
%According to their results, 
%the use of mention heads instead of maximum spans results in about two percent difference in evaluation scores,
%except for the Stanford rule-based system \cite{leeheeyoung11} for which the difference is about four percent.
\newcite{penghaoruo15} extract mention heads using Collins' head finder rules \cite{collins99b}.
They use gold constituency-based parse trees and gold named entity information.
The gold parse information is only used during training to train their mention head detection classifier.
The gold named entity information is used to specify the whole span of named entities as their heads.
The reason is that the head finding rules only specify one word as a head,
and one-word heads can be troublesome for named entities,
e.g.,\ ``Green'' would be selected as the head of both ``Mary Green'' and ``John Green''.

%Mention heads can also be considered as potential minimum spans.
%: head finding rules are designed to extract the most important word of mentions and for mentions with more than one word, they only contain a subset of words from the original maximum span.
In this paper, we also examine the use of head words as minimum spans.
We show that compared to head words, \mina spans are more compatible with expert annotated minimum spans.

Since we evaluate minimum spans on various corpora, from which some do not include gold named entity information or even gold parse trees,
we only use Collins' head finder rules, without the final adjustment for named entities, as the baseline for minimum span detection.

Collins' rules for finding the head of a noun phrase (NP) are as follows:
\squishlist
\item If the tag of the last word is POS, return it as the head,
\item else return the first child, from right to left, with an NN, NNP, NNPS, NNS, NX, POS, or JJR tag, if there is any,
\item else return the first child, from left to right, with an NP tag, if there is any,
\item else return the first child, from right to left, with one of the \$, ADJP, or PRN tags, if there is any,
\item else return the first child, from right to left, with a CD tag, if there is any,
\item else return the first child, from right to left, with a JJ, JJS, RB, or QP tag, if there is any,
\item else return the last word.
\squishend

For the head finder rules for phrases other than NPs, please refer to Appendix A of \newcite{collins99b}.

%Unlike the head finding rules used in \newcite{penghaoruo15}, \mina can use system parse trees and does not
%require named entity information.
%Besides, except for one word mentions, 
%extracted minimum spans by MINT are mainly longer than one word,
%e.g.\ all terminal nodes of all valid phrases that have the shortest distance to the root, including determiners and adjectives,
%are returned as the minimum span.

==> mina_acl2019/why.tex <==
\section{Why to Use Minimum Spans?}
\label{ch:min_span:why}


Example~\ref{} is an example 
\begin{figure}
\centering
 \resizebox{\columnwidth}{!}{\Tree [.VP establish [.NP [.NP a private bilingual school ] [.VP called [.S [.NP Little Oxford ]]]][.PP in [.NP [.NP February ][.NP 1998 ]]]]}
 \caption{Part of Example~\ref{pp_attachment_example} gold parse tree.\label{pp_attachment_example_gold}}
\end{figure}

\begin{figure}
\centering
 \resizebox{\columnwidth}{!}{\Tree [.NP [.NP a private bilingual school ][.VP called [.S [.NP Little Oxford ][.PP in [.NP February 1998 ]]]]]}
 \caption{Detected maximum span of Example~\ref{pp_attachment_example}.\label{pp_attachment_example_system}}
\end{figure}

Example~\ref{pp_attachment_example} is instances of such mismatches for which the corresponding parse trees are shown in Figure~\ref{pp_attachment_example_gold} and ~\ref{pp_attachment_example_system}.

Differences between gold annotated compared to their corresponding system detected mentions
are not limited to variations of PP-attachments.
An example of such variations is presented in Appendix~\ref{appendix-1}.
 
In each of such cased, 
any system that uses the provided system parse trees for detecting mention boundaries,
missed the resolution of the corresponding gold mentions, and potentially their coreferring mentions,
only because of parsing errors.

